Almost-Isometric Embeddings of Graphs into Riemannian Manifolds

Graphs represent objects as vertices and relationships as edges; positive edge weights define shortest-path metrics. Metric embeddings leverage target-space geometry to analyze distances. Foundational results target linear spaces: Nash embedded Riemannian manifolds isometrically into Euclidean space, and Bourgain embedded $n$-point metrics into Hilbert space with $O(\log n)$ distortion. By contrast, the manifold hypothesis places high-dimensional data near low-dimensional smooth manifolds, making such manifolds themselves target spaces. What distortion is needed to embed a finite graph metric into such a manifold with its intrinsic distance? Although the star $K_{1,3}$ cannot embed isometrically into any complete Riemannian manifold, we prove almost-isometric embeddings always exist: for $\varepsilon>0$ and any finite connected positively weighted graph, we construct a smooth connected closed orientable surface in $\mathbb{R}^3$ admitting a noncontractive $(1+\varepsilon)$-embedding of its vertices, with $\varepsilon$ arbitrarily small and independent of graph parameters. This construction transfers communication schemes between graphs and surfaces. For independent unicasts, fractional routing splits flows across paths while network coding lets relays combine messages. Space information flow permits relays anywhere, charging bandwidth times distance. Whereas coding advantage (optimal routing over coding cost) equals one in Euclidean space, we prove coding advantages on finite positively weighted undirected graphs transfer to smooth closed surfaces within factors approaching one. Counterexamples to the multiple-unicast conjecture and amplification yield smooth closed surfaces with unbounded coding advantage. Conversely, coding advantage is at most $C\log(g+2)$ on finite undirected graphs of orientable genus $g$ and smooth closed orientable surfaces of genus $g$, for absolute $C$.

==> figures/construction.tex <==
\begin{tikzpicture}[mf diagram]
% The example has four vertices and five edges. The named diagonal path
% is reused literally in (b) and (c), including the two straight collars.
\def\topology{(0,1.55) -- (2.88,1.90) -- (3.35,.02) -- (.56,-.48) -- cycle}
\def\wave{(0,0) -- (.66,0) .. controls (.86,0) and (.86,.27) .. (1.03,.27)
 .. controls (1.23,.27) and (1.23,-.27) .. (1.42,-.27)
 .. controls (1.61,-.27) and (1.61,.27) .. (1.80,.27)
 .. controls (1.99,.27) and (1.99,-.27) .. (2.18,-.27)
 .. controls (2.37,-.27) and (2.37,.25) .. (2.56,.25)
 .. controls (2.74,.25) and (2.76,0) .. (2.95,0) -- (3.68285,0)}
\tikzset{diagonal frame/.style={shift={(0,1.55)},rotate=-24.55}}
\def\plainvertices{\foreach \x/\y in {0/1.55,2.88/1.90,3.35/.02,.56/-.48}
  \node[mf vertex] at (\x,\y) {};}
\begin{scope}[shift={(.45,.32)}]
 \node[mf heading] at (-.34,2.72) {\mftext{(a) Straight embedding}{(a) 无交叉直线嵌入}};
 \draw[mf edge] \topology;
 \draw[mf edge] (0,1.55)--(3.35,.02);
 \plainvertices
 \node[above left=2pt] at (0,1.55) {$1$}; \node[above right=2pt] at (2.88,1.90) {$2$};
 \node[right=3pt] at (3.35,.02) {$3$}; \node[below left=2pt] at (.56,-.48) {$4$};
 \node at (1.65,-1.12) {$\Gamma_0\subset\mathbb R^3$};
\end{scope}
\draw[mf step] (4.45,1.13)--(5.20,1.13);
\begin{scope}[shift={(6.00,.32)}]
 \node[mf heading] at (-.50,2.72) {\mftext{(b) Prescribe arclengths}{(b) 调整空间边长}};
 \draw[mf edge] \topology;
 \begin{scope}[diagonal frame]
  \path[fill=mfPale!60] (.58,-.39) rectangle (3.03,.39);
  \draw[mf axis] (.58,0)--(3.03,0);
  \draw[mfBlue,dashed,line width=.68pt] (.58,.39)--(3.03,.39) (.58,-.39)--(3.03,-.39);
  \foreach \x in {.58,3.03}{\draw[mfBlue,dash pattern=on 1.6pt off 1.3pt,line width=.65pt] (\x,0) ellipse[x radius=.13,y radius=.39];}
  \draw[mfRust,line width=1.35pt] \wave;
 \end{scope}
 \plainvertices
 \node[text=mfBlue] (ze) at (1.83,2.03) {$Z_e$};
 \draw[mf lead] (ze.south)--(1.71,1.20);
 \node at (1.67,-1.12) {$L_e=(1+\eta)c_e$};
\end{scope}
\draw[mf step] (9.93,1.13)--(10.68,1.13);
\begin{scope}[shift={(11.40,.32)}]
 \node[mf heading] at (-.32,2.72) {\mftext{(c) Thicken the graph}{(c) 加粗得到曲面}};
 \mfTubeStroke{\topology}
 \begin{scope}[diagonal frame]\mfTubeStroke{\wave}\end{scope}
 \foreach \x/\y in {0/1.55,2.88/1.90,3.35/.02,.56/-.48}{\mfJoint{\x}{\y}}
 \node at (1.65,-1.12) {$g(M_r)=m-n+1$};
\end{scope}
\end{tikzpicture}


==> figures/tube-maps.tex <==
\begin{tikzpicture}[mf diagram]
\node[mf heading] at (0,6.25) {\mftext{(a) Geometry of a trimmed tube}{(a) 截短圆管的局部几何}};
\begin{scope}[shift={(3.50,4.44)},xscale=1.08]
 \mfLocalTube
 % The centerline lies in the plane of the spatial edge; the wall trace
 % is translated by a CONSTANT vector in the normal direction of that plane.
 \draw[mf axis] \mfArc;
 \draw[mf axis] (-.92,0)--(0,0) (8,0)--(8.92,0);
 \begin{scope}[shift={(.075,-.155)}]\draw[mfIndigo,line width=.95pt] \mfArc;\end{scope}
 \foreach \xx in {-.92,8.92}{
    \draw[mfEdge,line width=.55pt] (\xx-.052,-.052)--(\xx+.052,.052) (\xx-.052,.052)--(\xx+.052,-.052);}
 \node at (-.94,.24) {$U_u$}; \node at (8.92,.24) {$U_v$};
 \node[below] at (-.92,-.63) {$p_u$}; \node[below] at (8.92,-.63) {$p_v$};
 \node (core) at (2.24,1.21) {$\gamma_e(s)$};
 \draw[mf lead] (core.south)--(2.45,.419);
 \node[text=mfIndigo] (wall) at (5.77,1.24) {$X_e(s)=\gamma_e(s)+r w_e$};
 \draw[mf lead] (wall.south)--(5.35,.347);
 \node[text=mfBlue] (tube) at (7.62,.93) {$T_e$};
 \draw[mf lead] (tube.south)--(7.37,.34);
 % The vertical radius is measured at a straight collar, from axis to wall.
 \draw[mfRust,{Stealth[length=1.15mm]}-{Stealth[length=1.15mm]},line width=.55pt]
 (.41,0)--(.41,.33);
 \node[text=mfRust] (rad) at (.64,.74) {$r$};
 \draw[mf lead] (rad.south)--(.43,.34);
 \node[mf detail] (bend) at (4.02,-.24) {\mftext{inner side of bend}{弯管内侧}};
 \draw[mf lead] (bend.north)--(4,.35);
 % Interval markers below indicate the endpoints of the corresponding ARC,
 % not a Euclidean measurement of its chord.
 \foreach \xx in {0,8}{\draw[mf guide,densely dotted] (\xx,-.34)--(\xx,-1.07);}
 \draw[mf lead] (0,-.95)--(8,-.95) (0,-.87)--(0,-1.03) (8,-.87)--(8,-1.03);
 \node[fill=white] at (4,-.95) {\mftext{trimmed arclength}{截短后的弧长} $\ell_e$};
 \foreach \xx in {-.92,8.92}{\draw[mf guide,densely dotted] (\xx,-.95)--(\xx,-1.38);}
 \draw[mf lead] (-.92,-1.34)--(8.92,-1.34) (-.92,-1.26)--(-.92,-1.42) (8.92,-1.26)--(8.92,-1.42);
 \node[fill=white] at (4,-1.34) {\mftext{full spatial arclength}{整条空间边的弧长} $L_e$};
\end{scope}
\draw[mf guide] (0,2.63)--(15.7,2.63);
\node[mf heading] at (0,2.25) {\mftext{(b) Maps on an oriented edge}{(b) 定向边上的双向映射}};
\draw[mf guide] (7.78,1.83)--(7.78,-1.80);
\node at (3.74,1.69) {$\iota: |G|\to M_r$};
\node at (11.74,1.69) {$\pi: M_r\to |G|$};
% Left: full graph edge is parametrized at constant speed along lambda_e.
\draw[mf edge] (.78,1.00)--(6.73,1.00);
\foreach \xx/\lab in {.78/u,6.73/v}{\node[mf vertex] at (\xx,1.00) {};\node[above] at (\xx,1.06) {$\lab$};}
\node[mf mapped] at (3.74,1) {}; \node[above] at (3.74,1.04) {$x$};
\begin{scope}[shift={(1.25,-.65)},xscale=.62,yscale=.48]
 \mfLocalTube
 \draw[mfIndigo,line width=1.12pt] (-.93,-.14) .. controls (-.61,-.34) and (-.36,-.155) .. (.075,-.155);
 \begin{scope}[shift={(.075,-.155)}]\draw[mfIndigo,line width=1.12pt] \mfArc;\end{scope}
 \draw[mfIndigo,line width=1.12pt] (8.075,-.155) .. controls (8.38,-.18) and (8.57,-.36) .. (8.93,-.14);
 \foreach \x/\y in {-.93/-.14,4.075/.525,8.93/-.14}{\node[mf mapped] at (\x,\y) {};}
\end{scope}
\draw[mf forward] (3.74,.87)--(3.77,-.28) node[pos=.43,anchor=west] {$\iota$};
\node[mf detail,text=mfIndigo,above] at (5.16,-.43) {$\lambda_e$};
\node[below] at (.89,-.98) {$q_u=\iota(u)$};
\node[below] at (6.60,-.98) {$q_v=\iota(v)$};
\node[below,text=mfIndigo] at (3.77,-.57) {$\iota(x)$};
% Right: reserve separate rows for the map title, section callout and image.
\begin{scope}[shift={(9.27,.16)},xscale=.62,yscale=.48]
 \mfLocalTube
 \draw[mfRust,line width=1.15pt] (4,.68) ellipse[x radius=.17,y radius=.33];
\end{scope}
\node[mf detail] at (8.68,.16) {$U_u$};
\node[mf detail] at (14.82,.16) {$U_v$};
\node[text=mfRust,anchor=west,inner sep=0pt]
  (sectionlabel) at (12.56,1.06) {\mftext{section at fixed $s$}{固定 $s$ 的横截面}};
\draw[mf lead,draw=mfRust] (sectionlabel.west) ++(-.11,0)
  -- (12.25,1.06) -- (11.89,.70);
\draw[mf edge] (8.68,-1.09)--(14.82,-1.09);
\foreach \xx/\lab in {8.68/u,14.82/v}{
 \draw[mf back,densely dashed] (\xx,-.19)--(\xx,-.96);
 \node[mf vertex] at (\xx,-1.09) {};
 \node[below=4pt] at (\xx,-1.09) {$\lab$};}
\draw[mf back] (11.75,.24)--(11.75,-.95);
\node[mf relay] at (11.75,-1.09) {};
\node[below=5pt,text=mfRust] at (11.75,-1.09) {$c_e s/\ell_e$};
\end{tikzpicture}

